Pandemic Spread in Communities via Random Graphs

Working in the multi-type Galton-Watson branching-process framework we analyse the spread of a pandemic via a general multi-type random contact graph. Our model consists of several communities, and takes, as input, parameters that outline the contacts between individuals in distinct communities. Given these parameters, we determine whether there will be an outbreak and if yes, we calculate the size of the giant connected component of the graph, thereby, determining the fraction of the population of each type that would be infected before it ends. We show that the pandemic spread has a natural evolution direction given by the Perron-Frobenius eigenvector of a matrix whose entries encode the average number of individuals of one type expected to be infected by an individual of another type. The corresponding eigenvalue is the basic reproduction number of the pandemic. We perform numerical simulations that compare homogeneous and heterogeneous spread graphs and quantify the difference between them. We elaborate on the difference between herd immunity and the end of the pandemic and the effect of countermeasures on the fraction of infected population.

==> preamble.tex <==
%--------------
%% preamble.tex
%% this should be included with a command like
%% \input{preamble.tex}


\usepackage[utf8]{inputenc}
%\usepackage{draftcopy}
%\usepackage{draftwatermark}

%%%%%%% Muli commands %%%%



\usepackage{graphicx}
\usepackage{fullpage}

\usepackage{amssymb}

\usepackage{amsmath}

\usepackage{amsthm}

\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}

\newcommand\comment[1]{\fbox{\tt #1}}

\newcommand\subspaces[2] { \genfrac[]{0pt}{}{#1}{#2} }

%\usepackage{algorithm}
%\usepackage[noend]{algpseudocode}
%\renewcommand{\algorithmicrepeat}{}
%\renewcommand{\algorithmicuntil}{}
%\renewcommand{\algorithmicif}{\textbf{If}}
%\renewcommand{\algorithmicelse}{\textbf{Else }}
%\renewcommand{\algorithmicloop}{}
%\renewcommand{\algorithmicfor}{\textbf{For}}




\newtheorem{theorem}{Theorem}[subsection]
   \newtheorem{thm}{Theorem}[subsection]
   \newtheorem{conj}[thm]{Conjecture}
   \newtheorem{lemma}[theorem]{Lemma}
   \newtheorem{corollary}[thm]{Corollary}
   \newtheorem{claim}[theorem]{Claim}
   \newtheorem{proposition}[thm]{Proposition}
   \newtheorem{definition}[theorem]{Definition}
   \newtheorem{remark}[theorem]{Remark}
    \newtheorem{fact}{Fact}
    \newtheorem{assumption}{Assumption}
    \newtheorem{observation}{Observation}

%\newcommand\gap{ \textsf{gap-} }
%\newcommand\gapV{ \textsf{gap$_V$-} }

\newcommand\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\Z{\mathbb{Z}}

\newcommand\card[1]{\left| {#1} \right|}

\newcommand\tup[1]{\left\langle #1 \right\rangle}

\newcommand\set[1]{{\left\{ #1 \right\}}}
\newcommand\Set[2]{ \left\{ #1 \vert #2\right\} }
\newcommand\sett[2]{\left\{ \left. #1 \;\right\vert #2 \right\}}
\newcommand\settright[2]{\left\{ #1 \;\left\vert\; #2 \right.\right\}}

\newcommand\Prob[2]{{\Pr_{#1}\left[ {#2} \right]}}
\newcommand\cProb[3]{{\Pr_{#1}\left[ \left. #3 \;\right\vert #2 \right]}}
\newcommand\cProbright[3]{{\Pr_{#1}\left[ #3\;\left\vert  #2\right. \right]}}
\newcommand\Expect[2]{{\mathop{\mathbb{E}}_{#1}\left[ {#2} \right]}}
\newcommand\cExpect[3]{{\mathbb{E}_{#1}\left[ \left. #3 \;\right\vert #2 \right]}}

\newcommand\ang[1]{\langle {#1}\rangle}

\newcommand\norm[1]{\| #1 \|}

\newcommand\power[1]{\set{0,1}^{#1}}

\newcommand\ceil[1]{\lceil{#1}\rceil}

\newcommand\round[1]{\left\lfloor{#1}\right\rfloor}

\newcommand\half{\frac{1}{2}}
\newcommand\quarter{\frac{1}{4}}
\newcommand\eigth{\frac{1}{8}}

\newcommand\defeq{\stackrel{def}{=}}

\newcommand\skipi{{\vskip 10pt}}

\newcommand\IP[2]{\left\langle {#1}, {#2} \right\rangle}
\newcommand\inner[2]{\left\langle{#1},{#2}\right\rangle}

\newcommand\TF{ {\set{T, F}} }
\newcommand\pmo{ { \{\pm 1\} } }
\newcommand\Gn{ {\pmo^n} }
\newcommand\BF{ {\colon\Gn\to\pmo } }
\newcommand\cube[1]{ { \set{-1,1}^{#1} } }

\newcommand\nV{{\cal \#V}}
\newcommand\pV{{ p{\cal V} }}
\newcommand\tV{ {\cal \widetilde{V} } }

\newcommand\sqrtn{ {\sqrt n} }
\newcommand\eps{\epsilon}

\newcommand\minimum[2] {  \min\left\{{{#1}, {#2}}\right\}   }

\newcommand\spn{span}
\newcommand\spnn[1]{span({#1})}

\newcommand\Ext{{\sf s-Ext}}

\newcommand\Extt{{\sf Ext}}

\newcommand\sgn[1]{sign({#1})}

\newcommand*\xor{\mathbin{\oplus}}

\newcommand*\bxor{\mathbin{\bigoplus}}

\newcommand*\Hell[2]{{H\left({#1}, \ {#2}\right)}}

\newcommand*\cHell[4]{{H\left({#1}\vert({#2}),\ {#3}\vert({#4}) \right)}}

\newcommand*\QED{}

\newcommand*\Uni{{\cal U}}

%%%%%%% \end{Muli commands} %%%%
%%%%%%% \begin{Esty commands} %%%%
   \newtheorem{untruth}[thm]{Untruth}

\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}

\newcommand*\entropy{ {\cal H} }

\newcommand\parentheses[1]{{\left({#1}\right)}}
\newcommand\ps[1]{\parentheses{#1}}

\newcommand\brackets[1]{{\left[{#1}\right]}}
\newcommand\fcoefficient[2]{{\widehat{#1}\parentheses{#2}}}

\newcommand\sqfcoefficient[2]{{\widehat{#1}^2\parentheses{#2}}}

\newcommand\fchar[1]{{\chi_{#1}}}


\newcommand\pentropy[1]{{\entropy\brackets{#1}}}
\newcommand\hentropy[1]{\entropy_\half\brackets{#1}}
\newcommand\parentropy[1]{\entropy_p\brackets{#1}}
%charcters entropy
\newcommand\charentropy[1]{{\pentropy{\widehat{#1}^2}}}
\newcommand\charhentropy[1]{{\hentropy{\widehat{#1}^2}}}
%values entropy
\newcommand\valentropy[1]{{\pentropy{{#1}^2}}}

\newcommand\plog[1]{{\log\parentheses{#1}}}
\newcommand\pln[1]{{\ln\parentheses{#1}}}
\newcommand\pfrac[2]{{\parentheses{\frac{#1}{#2}}}}

% Symmetric difference of sets%
\newcommand\symdif{\vartriangle}

%function degree%
\newcommand\fdeg[1]{{deg\parentheses{#1}}}

%absolute value%
\newcommand\abs[1]{{\left\lvert{#1}\right\rvert}}


%TODO list%
\usepackage{soul}
\usepackage{xcolor}
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\technical[1]{\textcolor{gray}{#1}}
\newcommand\purple[1]{\textcolor{purple}{#1}}
\newcommand\yellow[1]{\textcolor{yellow}{#1}}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\assume[1]{\textcolor{orange}{#1}}
\newcommand\green[1]{\textcolor{green!40!black}{#1}}

%some macroes%
%alpha fraction for: %
\newcommand\idxalpha[2]{{\alpha_{#2}}}
%derivative%
\newcommand\fInduct[2]{f_{{#1}({#2})}}
\newcommand\fD[1]{\fInduct{D}{#1}}
\newcommand\fDj{\fD{j}}
\newcommand\fA[1]{\fInduct{A}{#1}}
\newcommand\fAj{\fA{j}}
\newcommand\alphaD[1]{{\alpha_{#1}}}
\newcommand\alphaDj{\alphaD{j}}
\newcommand\fIndcutUpper[2]{f^{{#1}({#2})}}
\newcommand\fsigmaj{\fIndcutUpper{\sigma}{j}}
\newcommand\fpmsi[3]{{#1}^{{#2}({#3})}}
\newcommand\fpi[2]{\fpmsi{#1}{+}{#2}}
\newcommand\fmi[2]{\fpmsi{#1}{-}{#2}}
\newcommand\fsi[2]{\fpmsi{#1}{\sigma}{#2}}
\newcommand\fpj[1]{\fpi{#1}{j}}
\newcommand\fmj[1]{\fmi{#1}{j}}
\newcommand\fsj[1]{\fsi{#1}{j}}
\newcommand\fplus[1]{f^{+({#1})}}
\newcommand\fminus[1]{f^{-({#1})}}
\newcommand\fminusj{\fminus{j}}
\newcommand\fplusj{\fplus{j}}
\newcommand\betaj{\beta_j}
\newcommand\deltaj{\delta_j}
\newcommand\M[1]{{M\brackets{#1}}}
\newcommand\p[1]{{p\brackets{#1}}}
\newcommand\dkl[2]{D_{KL}\brackets{{#1},{#2}}}
\newcommand\dfu[1]{\dkl{#1}{U_{2^n}}}
\newcommand\SD[2]{SD\brackets{{#1},{#2}}}
\newcommand\pnorm[1]{{\norm{{#1}}_\p{{#1}}}}
\newcommand\gparam[1]{{\gamma\brackets{{#1}}}}
\newcommand\gpparam[2]{{\gamma_{#1}\brackets{{#2}}}}
\newcommand\noisyf[2]{T_{#1}[{#2}]}
\newcommand\frho{T_\rho[f]}

\newcommand\fDi{\partial_if}
%\renewcommand\betaj{{\frac{\half\norm{\fminusj}_2^2}{\norm{f}_2^2}}}
\newcommand\oneminusbetaj{{\frac{\half\norm{\fplusj}_2^2}{\norm{f}_2^2}}}
%\renewcommand\alphaDj{{\frac{\norm{\fDj}_2^2}{\norm{f}_2^2}}}

\renewcommand\fDj{\partial_jf}

\renewcommand\fminusj{{f^-}}
\renewcommand\fplusj{{f^+}}
%average%



%moments%
%second moment%
\newcommand\secmoment[2]{\Expc{{#2}\sim\Lambda {#1}}{|{#2}|^2}}
%first moment%
\newcommand\firstmoment[2]{\Expc{{#2}\sim\Lambda {#1}}{|{#2}|}}

%norms%
\newcommand\snorm[2]{\brokenvert\brokenvert{#2}\brokenvert\brokenvert_{#1}}
\newcommand\enorm[2]{\norm{#2}_{#1}}

\usepackage{wasysym}
\usepackage{comment}
\usepackage{marvosym}
%\usepackage{bbold}
%\usepackage{breqn}



%log of norm relations
\newcommand\logparama[2]{{\log\frac{\norm{#2}_2}{\norm{#2}_{#1}}}}
\newcommand\logparam[1]{{\log\frac{\norm{#1}_2}{\norm{#1}_1}}}
\newcommand\logparamp[1]{\logparama{p}{#1}}


\newcommand\indicator[1]{{\mathbb 1}_{#1}}
%%%%%%% \end{Esty commands} %%%%

